Privacy against Statistical Matching: Inter-User Correlation

Modern applications significantly enhance user experience by adapting to each user's individual condition and/or preferences. While this adaptation can greatly improve utility or be essential for the application to work (e.g., for ride-sharing applications), the exposure of user data to the application presents a significant privacy threat to the users, even when the traces are anonymized, since the statistical matching of an anonymized trace to prior user behavior can identify a user and their habits. Because of the current and growing algorithmic and computational capabilities of adversaries, provable privacy guarantees as a function of the degree of anonymization and obfuscation of the traces are necessary. Our previous work has established the requirements on anonymization and obfuscation in the case that data traces are independent between users. However, the data traces of different users will be dependent in many applications, and an adversary can potentially exploit such. In this paper, we consider the impact of correlation between user traces on their privacy. First, we demonstrate that the adversary can readily identify the association graph, revealing which user data traces are correlated. Next, we demonstrate that the adversary can use this association graph to break user privacy with significantly shorter traces than in the case when traces are independent between users, and that independent obfuscation of the data traces is often insufficient to remedy such. Finally, we discuss how the users can employ dependency in their obfuscation to improve their privacy.

==> framework-4.tex <==
\section{Framework}
\label{sec:framework}
Here, we employ a similar framework to~\cite{tifs2016,ISIT17}. In this framework, there is a system with $n$ users where $X_u(k)$ is the sample of the data of user $u$ at time $k$. Our main goal is protecting $X_u(k)$ from a strong adversary $(\mathcal{A})$ who has full knowledge of the marginal probability distribution function of all users based on the previous observations or other resources. In order to achieve data privacy of users, both anonymization and obfuscation techniques can be used as shown in  Figure \ref{fig:xyz}. In Figure \ref{fig:xyz}, $\widehat{X}_u(k)$ shows the (reported) sample of the data of user $u$ at time $k$ after applying obfuscation, and $\widetilde{X}_u(k)$ shows the (reported) sample of the data of user $u$ at time $k$ after applying anonymization. The adversary tries to estimate $X_u(k)$, $k=1, 2, \cdots, m$,  by obtaining $m$ observations per user. As we will see, $m=m(n)$ shows the number of data points after which the pseudonyms of users are changed in the anonymization method.

\begin{figure}[h]
	\centering
	\includegraphics[width = 1\linewidth]{fig/xyz}
	\caption{Applying obfuscation and anonymization techniques to users' data samples.}
	\label{fig:xyz}
\end{figure}



$\textbf{X}_u^{(n)}$ is the  $m \times 1$ vector containing the sample of the data of user $u$, and $\textbf{X}^{(n)}$ is the $m \times n$ matrix with $u^{th}$ column equal to $\textbf{X}_u^{(n)}$;
\[\textbf{X}_u^{(n)} =\left [
X_u(1), X_u(2) , \cdots,X_u(m\right]^T \]
\[ \textbf{X}^{(n)} =\left[\textbf{X}_{1}^{(n)}, \textbf{X}_{2}^{(n)}, \cdots,  \textbf{X}_{n}^{(n)}\right].
\]



\textit{Data Samples Model:}
We assume users' data samples can have $r$ possibilities $(0, 1, \cdots, r-1)$. Thus, according to a user-specific probability distribution, $X_u(k)$ is equal to a value in $\left\{0,1, \cdots, r-1 \right\}$ at any time, and these user-specific probability distributions are known to the adversary $(\mathcal{A}).$

\textit{Association Graph:}
A association graph or dependency graph is an undirected graph representing dependencies of users towards each other. $G(V,E)$ denotes the association graph where $V$ is the set of nodes $(|V|=n)$ of this graph, and E is the set of edges of this graph. Two vertices (users) are connected, if their data sets are dependent. More specifically,
\begin{itemize}
	\item $(i,j) \in E$ if $I(X_i(k); X_j(k))>0,$
	\item $(i,j) \notin E$ if $I (X_i(k);X_j(k))=0,$
\end{itemize}
where $I(X_i(k); X_j(k))$ is the mutual information between user $X_i(k)$ and user $X_j(k)$.

\textit{Obfuscation Model:} In obfuscation technique, the users' data samples are perturbed. Each user has only limited knowledge of the characteristics of the overall population, so usually a simple distributed method in which the samples of the data of each user are reported with error with a certain probability is employed. Note, this probability itself is generated randomly for each user.  Let $\widehat{\textbf{X}}_u^{(n)}$ be the vector which contains
%$m$ number of
the obfuscated versions of user $u$'s data sample, and $\widehat{\textbf{X}}^{(n)}$ is the collection of $\widehat{\textbf{X}}_u^{(n)}$ for all users,

Here we would like to define the \emph{asymptotic noise level} for an obfuscation technique. Loosely speaking, the asymptotic noise level of obfuscation is the highest probable percentage of data points that are corrupted. Let $X_u(k)$ be the actual sample of the data of user $u$ at time $k$, $u \in \{1, 2, \cdots, n'\}$, $k \in \{1, 2, \cdots, m\}$ and let $\widehat{X}_u(k)$ be the obfuscated (noisy) version of $X_u(k)$. Define
 \[A_m(u) = \frac{\abs{\left\{k:\widehat{X}_u(k) \neq X_u(k)\right\}}}{m},\]
 then asymptotic noise level for user $u$ is defined as follows:
 \[a (u)=\inf \bigg\{ a \geq 0: P(A_m(u)>a) \rightarrow 0 \text{ as }  m \rightarrow \infty\bigg\}.\]

 Also define
 \[A_m= \frac{\sum\limits_{u=1}^{n'} \abs{\left\{k:\widehat{X}_u(k) \neq X_u(k)\right\}}}{mn'},\]
 then the asymptotic noise level for the entire data set is
 \[a =\inf \bigg\{ a \geq 0: P(A_m>a) \rightarrow 0 \text{ as }  m \rightarrow \infty\bigg\}.\]
 Note while the above definition is given for a general case, in practice usually we use simple obfuscation techniques that are given by $i.i.d.$ noise sequences. Therefore, by using the Strong Law of Large Number (SLLN),
 \[\frac{\abs{\left\{k:\widehat{X}_u(k) \neq X_u(k)\right\}}}{m} \xrightarrow{\text{a.s.}} P\left(\widehat{X}_u(k) \neq X_u(k)\right).\]
Thus, we usually have
\[a(u)=P\left(\widehat{X}_u(k) \neq X_u(k)\right).\]


\textit{Anonymization Model:} In the anonymization technique, the identity of the users is perturbed. Anonymization is modeled by a random permutation $\Pi$ on the set of $n$ users. Let $\widehat{\textbf{X}}_u^{(n)}$ be the vector which contains the anonymized version of $\widetilde{\textbf{X}}_u^{(n)}$, and $\widetilde{\textbf{X}}^{(n)}$ is the collection of $\widetilde{\textbf{X}}_u^{(n)}$ for all users, thus $\widetilde{\textbf{X}}_{u}^{(n)} = \widehat{\textbf{X}}_{\Pi^{-1}(u)}^{(n)}$ and $\widetilde{\textbf{X}}_{\Pi(u)}^{(n)} = \widehat{\textbf{X}}_{u}^{(n)}$.


\textit{Adversary Model:} We consider the strongest reasonable adversary that has has full knowledge of the marginal probability distribution function of all users through past observations or some other sources. The adversary knows the probability distribution for each user on the set of data samples $\{0,1,\ldots,r-1\}$. The adversary also knows the anaonymization mechanism, but does not know the realization of the random permutation. The adversary knows the obfusaction mechanism, but does not know the realization of the noise parameters. Also, the adversary  knows the association graph $G(V,E)$, but does not necessarily know the exact nature of dependency. That is, while the adversary knows the marginal distributions $X_i(k)$ as well as which pairs of users have strictly positive mutual information, he might not know the joint distributions or even the values of mutual informations $I(X_i(k); X_j(k))$.

In \cite{tifs2016}, perfect privacy is defined as follows:
\begin{define}
User $u$ has \emph{perfect privacy} at time $k$, if and only if
\begin{align}%\label{}
\no  \forall k\in \mathbb{N}, \ \ \ \lim\limits_{n\rightarrow \infty} I \left(X_u(k);{\widetilde{\textbf{X}}^{(n)}}\right) =0,
\end{align}
where $I\left(X_u(k);{\widetilde{\textbf{X}}^{(n)}}\right)$ denotes the mutual information between a sample of the data of user $u$ at time $k$ and collection of adversary's observations for all the users.
\end{define}

\noindent In \cite{ISIT17}, the situation in which there is no privacy is also considered as follows:

\begin{define}
User $u$ has \emph{no privacy} at time $k$, if and only if there exists an algorithm for the adversary to estimate $X_u(k)$ perfectly as $n$ goes to infinity. In other words, as $n \rightarrow \infty$,
\begin{align}
\no  \forall k\in \mathbb{N}, \ \ \ P_e(u)\triangleq P\left(\overbrace{X_u(k)} \neq X_u(k)\right)\rightarrow 0,
\end{align}
where $\overbrace{X_u(k)}$ is the estimated value of $X_u(k)$ by the adversary.
\end{define}


\section{Impact of Correlation on Privacy Using Anonymization}
\label{anon}
In this section, the anonymization technique only employed to achieve privacy as shown in Figure \ref{fig:xy}.
In this figure, $\widetilde{{X}}_u(k)$ shows the (reported) sample of the data of user $u$ at time $k$ after applying anonymization. We have $\widetilde{\textbf{X}}^{(n)}$ which is the anonymized version of $\textbf{X}_u^{(n)}$; thus
$\widetilde{\textbf{X}}_{u}^{(n)} = {\textbf{X}}_{\Pi^{-1}(u)}^{(n)}$ and $\widetilde{\textbf{X}}_{\Pi(u)}^{(n)} = {\textbf{X}}_{u}^{(n)}$.

\begin{figure}[h]
	\centering
	\includegraphics[width = 0.7\linewidth]{fig/xy}
	\caption{Applying the anonymization technique to users' data samples.}
	\label{fig:xy}
\end{figure}

\subsection{$i.i.d.$ Two-State Model}
\label{iidtwo}

We first consider the $i.i.d.$ two-state $(r=2)$ case. For this case, the sample of the data of user $u$ at any time is a Bernoulli random variable with parameter $p_u$, which is the probability of user $u$ being at state $1$. Thus,
\[X_u(k) \sim Bernoulli \left(p_u\right).\]
The parameters $p_u$, $u=1, 2, \cdots, n$ are drawn independently from a continuous density function, $f_P(p_u)$, on the $(0,1)$ interval. The density $f_P(p_u)$ might be unknown, so all it is assumed here is that such density exists. From the results of the paper, it will be evident that knowing or not knowing $f_P(p_u)$ does not change the results asymptotically.  Further, we assume there are $\delta_1, \delta_2>0$ such that\footnote{The condition $\delta_1<f_P(p_u) <\delta_2$ is not actually necessary for the results and can be relaxed; however, we keep it here to avoid unnecessary technicalities.}:
\begin{equation}
\no\begin{cases}
    \delta_1\leq f_P(p_u) \leq\delta_2, & p_u \in (0,1).\\
    f_P(p_u)=0, &  p _u\notin (0,1).
\end{cases}
\end{equation}

The adversary knows the values of $p_u$, $u=1, 2, \cdots, n$ and uses this knowledge to identify users. We will use capital letters (i.e., $P_u$) when we are referring to the random variable, and use lower case (i.e., $p_u$) to refer to the realization of $P_u$.

A vector containing the permutation of those probabilities after anonymization is $\widetilde{\textbf{P}}$ , where $\widetilde{P}_{u} = {{P}}_{\Pi^{-1}(u)}$ and  $\widetilde{P}_{\Pi(u)} = {{P}}_{u}$. As a result,  for $u=1,2,..., n$, the distribution of the data symbols for the user with pseudonym $u$ is given by:
\[ \widetilde{X}_u^{(n)}(k) \sim Bernoulli \left(\widetilde{P}_u\right) \sim Bernoulli\left(P_{\Pi^{-1}(u)}\right)  .\]

For this case, dependency and correlation of data samples are equivalent, that is, we can say:
\begin{itemize}
	\item $(i,j) \in E$ if $\rho (X_i(k),X_j(k))=\rho_{ij}>0,$
	\item $(i,j) \notin E$ if $\rho (X_i(k),X_j(k))=\rho_{ij}=0,$
\end{itemize}
where $\rho_{ij}$ is the correlation coefficient between user $i$ and user $j$. The adversary knows the association graph $G(V,E)$, but does not necessarily know the correlation coefficient $(\rho_{ij})$ for each specific $(i,j) \in E$.


The following lemma states that if $m=m(n)$ is significantly larger than or equal to $(\log n)^3$ in this two-state model, then the adversary can reconstruct the entire association graph for \textit{the anonymized version of data} with vanishing error probability.
\begin{lem}
	\label{lem1}
	Consider a general association graph $G(V,E)$. If the adversary obtains $m=(log n)^3$ anonymized observations per user, he/she can construct $\widetilde{G}=\widetilde{G}(\widetilde{V}, \widetilde{E})$, where $\widetilde{V}=\{\Pi(i):i \in V\}=V$, such that for all $i, j \in V$; $ (i,j)\in E$ iff  $\left(\Pi(i),\Pi(j)\right)\in \widetilde{E}$. We write this statement as $P(\widetilde{E}=E)\rightarrow 1$.
\end{lem}


Knowing  the structure of the association graph $(G)$ leaks a lot of information.
For example, in Figure \ref{fig:identity}, the identity map is the only automorphism of the association graph $G$.  Thus, it is obvious that the adversary can uniquely identify users if he/she reconstruct the association graph.


To be able to derive further results, we need to make some assumptions on the structure of the association graph. For the rest of the paper, we consider a graph structure shown in Figure \ref{fig:graph}, where the association graph consists of $f$ disjoint subgraphs,
\[G=G_1 \cup G_2 \cup \cdots \cup  G_f,\]
where subgraph $G_i$, is a connected graph on $s_i$ vertices. In particular, each subgraph $G_i$ refers to a group of ``friends'' or ``associates'' such that their data sets are dependent. So we can write $G_i(V_i, E_i)$, where $|V_i|=s_i$.
\begin{figure}
	\centering
	\includegraphics[width=.6\linewidth]{fig/identity.jpg}
	\centering
	\caption{One example of association graph that the identity map is the only automorphism of that.}
	\label{fig:identity}
\end{figure}
\begin{figure}
	\centering
	\includegraphics[width=.5\linewidth]{fig/graph.jpg}
	\centering
	\caption{Association graph consists of some disjoint subgraphs $(G_i)$, where $G_i$ is a connected graph on $s_i$ vertices.}
	\label{fig:graph}
\end{figure}

The following theorem states that if the number of observations per user $(m)$ is significantly larger than $n^{\frac{2}{s}} $ in this two-state model, then the adversary can successfully de-anonymize the users.

\begin{thm}\label{two_state_thm}
For the above two-state model, if $\widetilde{\textbf{X}}^{(n)}$ is the anonymized version of $\textbf{X}^{(n)}$  as defined above, the size of a group is $s$, and
\begin{itemize}
	\item $m=cn^{\frac{2}{s}+\alpha}$, where $\alpha > 0$;
\end{itemize}
Then the adversary will be able to single out all members with arbitrary small error probability for large enough $n$. That is, as $n \rightarrow \infty$,
\begin{align}
\no  \forall k\in \mathbb{N}, \ \ \ P_e(1)\triangleq P\left(\overbrace{X_1(k)} \neq X_1(k)\right)\rightarrow 0.
\end{align}
\end{thm}

\textit{Discussion}:
Before proving the theorem, it is insightful to compare this result to Theorem 1 in \cite{tifs2016}. In that Theorem, it is stated that if the users are not correlated, then all users have perfect privacy as long as the number of adversary's observations per user $(m)$ is smaller than $O(n^2)$. Here, Theorem \ref{two_state_thm} states that with much smaller $m$ the adversary can de-anonymize all users. Therefore, we see that correlation can significantly reduce the privacy of users.
$\\$

\noindent \textbf{Proof of Theorem \ref{two_state_thm}:}
\begin{proof}
The proof of Theorem \ref{two_state_thm} (provided in the extended version \cite{ISIT18-longversion}) consists of three parts:
\begin{enumerate}
\item Showing the adversary can reconstruct the association graph with small error probability.
\item Showing the adversary can uniquely identify group $1$ with small error probability.
\item Showing the adversary can individually identify all the members within group $1$.
\end{enumerate}
\end{proof}


\subsection{$i.i.d.$ $r$-States Model}
\label{iidr}
Now, assume users' data samples can have $r$ possibilities $\left(0, 1, \cdots, r-1\right)$, and $p_u(i)$ shows the probability of user $u$ having data sample $i$.  We define the vector $\textbf{p}_u$ as% and the matrix $\textbf{P}$ as
\[\textbf{p}_u= [
p_u(1) ,  p_u(2) ,  \cdots, p_u(r-1) ]^T, \ \ \  \textbf{P} =\left[ \textbf{p}_{1}, \textbf{p}_{2}, \cdots,  \textbf{p}_{n}\right].
\]

We also assume $\textbf{p}_u$'s are drawn independently from some continuous density function, $f_P(\textbf{p}_u)$, which has support on a subset of the $(0,1)^{r-1}$ hypercube. In particular, define the range of distribution as
\begin{align}
\no  R_{\textbf{P}} &= \left\{ (x_1, \cdots, x_{r-1}) \in (0,1)^{r-1}: x_i > 0 , x_1+x_2+\cdots+x_{r-1} < 1\right\}.
\end{align}
Then, we assume there are $\delta_1, \delta_2>0$ such that:
\begin{equation}
\begin{cases}
\no    \delta_1\leq f_{\textbf{P}}(\mathbf{p}_u) \leq \delta_2, & \textbf{p}_u \in R_{\textbf{P}}.\\
    f_{\textbf{P}}(\mathbf{p}_u)=0, &  \textbf{p}_u \notin R_{\textbf{P}}.
\end{cases}
\end{equation}

\begin{thm}\label{r_state_thm}
For the above two-state model, if $\widetilde{\textbf{X}}^{(n)}$ is the anonymized version of $\textbf{X}^{(n)}$  as defined above, the size of a group is $s$, and
\begin{itemize}
	\item $m=cn^{\frac{2}{(r-1)s}+\alpha}$, where $\alpha > 0$;
\end{itemize}
then the adversary will be able to single out all members of the group with arbitrary small error probability for large enough $n$. That is as $n \rightarrow \infty$,
\begin{align}
\no  \forall k\in \mathbb{N}, \ \ \ P_e(1)\triangleq P\left(\overbrace{X_1(k)}  \neq X_u(k)\right)\rightarrow 0.
\end{align}
\end{thm}



\subsection{Markov Chain Model}
\label{markov}
In Sections \ref{iidtwo} and \ref{iidr}, we assumed users' data patterns are $i.i.d.$, however, in this section users' data patterns are modeled using Markov chains in which each user's data samples are dependent over time. In this model, we again assume there are $r$ possibilities for each data point, i.e., $X_u(k) \in \{0,1,2, \cdots, r-1\}$.

More specifically, each user's data is modeled by a Markov chain with $r$ states. It is assumed that the Markov chains of all users have the same structure, but have different transition probabilities. Let $F$ be the set of edges in the assumed transition graph, so $(i, j) \in F$ if there exists an edge from state $i$ to state $j$ meaning that $p_u(i,j)=P\left(X_u(k+1)=j|X_u(k)=i\right)>0$. Transition matrix is a square matrix used to describe the transitions of a Markov chain, thus different users can have different transition probability matrices. Note for each state $i$, we have
$\sum\limits_{j=1}^{r} p_u(i,j)=1,$
so the adversary can focus on a subset of size $d=|F|-r$ of transition probabilities for recovering the entire transition matrix.
So we have
\[\textbf{p}_u= [
p_u(1), p_u(2), \cdots, p_u(d) ]^T, \ \ \  \textbf{P} =\left[ \textbf{p}_{1}, \textbf{p}_{2}, \cdots,  \textbf{p}_{n}\right].
\]

We also consider $p_u(i)$'s are drawn independently from some continuous density function, $f_P(\textbf{p}_u)$, on the $(0,1)^{|F|-r}$ hypercube. Define the range of distribution as
\begin{align}
\no  R_{\textbf{P}} &= \left\{ (x_1, \cdots, x_{d}) \in (0,1)^{d}: x_i > 0 , x_1+x_2+\cdots+x_{d} < 1\right\}.
\end{align}

As before, we assume there are $ \delta_1, \delta_2 >0$, such that
\begin{equation}
\begin{cases}
\no   \delta_1\leq f_{\textbf{P}}(\textbf{p}) \leq \delta2 & \textbf{p} \in R_{\textbf{p}}\\
f_{\textbf{P}}(\textbf{p})=0 &  \textbf{p} \notin R_{\textbf{p}}
\end{cases}
\end{equation}



\begin{thm}\label{markov_thm}
	For the an irreducible, aperiodic Markov chain model, if $\widetilde{\textbf{X}}^{(n)}$ is the anonymized version of $\textbf{X}^{(n)}$  as defined above, the size of a group is $s$, and
	\begin{itemize}
		\item $m=cn^{\frac{2}{s(|F|-r)}+\alpha}$, where $\alpha > 0$;
	\end{itemize}
	then the adversary will be able to single out all members of the group with arbitrary small error probability for large enough $n$. That is as $n \rightarrow \infty$,
	\begin{align}
	\no  \forall k\in \mathbb{N}, \ \ \ P_e(1)\triangleq P\left(\overbrace{X_1(k)} \neq X_u(k)\right)\rightarrow 0.
	\end{align}
\end{thm}



\section{Privacy using Anonymization and Obfuscation}
\label{obfs}
Here, both anonymization and obfuscation techniques are employed to achieve privacy. As shown in Figure \ref{fig:xyz}, $\widehat{X}_u{(k)}$ shows the (reported) sample of the data of user $u$ at time $k$ after applying obfuscation, and $\widetilde{X}_u(k)$ shows the (reported) sample of the data of user $u$ at time $k$ after applying anonymization. We assume similar obfuscation to \cite{ISIT17}.







\subsection{$i.i.d.$ Two-State Model}
\label{iidtwo_obfs}
Again, let us start with the simplest case: $i.i.d.$ two-state model. As before, we assume that $p_u$'s are drawn independently from some continuous density function, $f_P(p_u)$, on the $(0,1)$ interval.

To create a noisy version of data samples, for each user $u$ we independently generate a random variable $R_u^{(n)}$ that is uniformly distributed between $0$ and $a_n$\footnote{The uniform distribution assumption for $R_u^{(n)}$ is not necessary and the results can be extended to a general set of distributions when we employ $\frac{a_n}{2}=E[R_u^{(n)}]$. However, the assumption of a uniform random variable simplifies the presentation of the results significantly.}. The value of $R_u^{(n)}$ shows the probability that the user's data sample is changed to a different value by obfuscation, and $a_n$ is termed the ``noise level'' of the system.

Note that the effect of the obfuscation is to alter the probability distribution function of each user across the $r$ possibilities in a way that is unknown to the adversary, since it is independent of all past activity of the user, and hence the obfuscation inhibits user identification. For each user, $R_u^{(n)}$ is generated once and is kept constant for the collection of samples of length $m$, thus providing a very low-weight obfuscation algorithm.



Note $\widehat{X}_u(k)$'s are $i.i.d.$ with a Bernoulli distribution because $X_u(k)$ are $i.i.d.$ and have a Bernoulli distribution, So we can say
\[\widehat{X}_u(k) \sim Bernoulli\left(\widehat{p}_u\right),\]
where $\widehat{p}_u$ is is the probability that an obfuscated data sample of user $u$ is equal to one, so
\begin{align}
\no \widehat{p}_u &=p_u(1-R_u^{(n)})+(1-p_u)R_u^{(n)}  \\
\nonumber &= p_u+\left(1-2p_u\right)R_u^{(n)}. \ \
\end{align}
Now we can define the vector $\widehat{\textbf{p}}$ which contains all the obfuscated probabilities.
\[\widehat{\textbf{P}} =\left[\widehat{{p}}_1, \widehat{{p}}_2, \cdots, \widehat{{p}}_n\right],\]
and the vector containing the permutation of those probabilities after anonymization is $\widetilde{\textbf{P}}$. As a result,  for $u=1,2,..., n$,
\[ \widetilde{X}_u(k) \sim Bernoulli \left(\widetilde{p}_u\right).\]




\begin{thm}\label{two_state_thm_converse_obfs}
	For the above two-state mode, if $\widehat{\textbf{X}}^{(n)}$ is the obfuscated version of $\textbf{X}^{(n)}$, and $\widetilde{\textbf{X}}^{(n)}$ is the anonymized version of $\widehat{\textbf{X}}^{(n)}$  as defined, and
	\begin{itemize}
		\item $m =cn^{\frac{2}{s} +  \alpha}$ for $c>0$ and $\alpha>0$;
		\item $R_u^{(n)} \sim Uniform [0, a_n]$, where $a_n \triangleq c'n^{-\left(\frac{1}{s}+\beta\right)}$ for $c'>0$ and $\beta>\frac{\alpha}{4}$;
	\end{itemize}
	user $1$ has no privacy as $n$ goes to infinity. In other words, there exists an algorithm for the adversary to produce the estimation of ${X_1(k)} $ such that for large enough $n$,
	\begin{align}
	\no  \forall k\in \mathbb{N}, \ \ \ P_e(1)\triangleq P\left(\overbrace{X_1(k)} \neq X_1(k)\right)\rightarrow 0.
	\end{align}
\end{thm}


\textit{Discussion}:
Before proving the theorem, it is insightful to compare this result to Theorem $1$ in \cite{ISIT17} which employed both anonymization and obfuscation techniques to achieve perfect privacy. That Theorem stated if the users are not correlated, then all users have perfect privacy as long as the number of adversary's observations per user $(m)$ is smaller than $O(n^2)$ or the the noise level $(a_n)$ used to obfuscated the users' data samples is larger that $O(n^{-1})$. Here, Theorem \ref{two_state_thm_converse_obfs} states that with much smaller $m$ or much larger $a_n$ the adversary can de-anonymize and de-obfuscate all users with vanishing error probability. Therefore, we see that correlation can significantly reduce the privacy of users.

Also, note that the asymptotic noise level is zero in this case. Specifically, if $A_m(u) = \frac{\abs{\left\{k:\widehat{X}_u(k) \neq X_u(k)\right\}}}{m}$, then
\[E[A_m(u)]=E[A_m]= O\left(\frac{1}{n^{\frac{1}{s}+\beta}}\right) \rightarrow 0,\]
which implies that the asymptotic noise level is zero.
$\\$

\subsection{$i.i.d.$ $r$-States Model}
Now, assume users' data samples can have $r$ possibilities $\left(0, 1, \cdots, r-1\right)$. Similar to Section \ref{iidr}, we assume $\textbf{p}_u$'s are drawn independently from some continuous density function, $f_P(\textbf{p}_u)$, which has support on a subset of the $(0,1)^{r-1}$ hypercube. $\textbf{p}_u$, $f_P(\textbf{p}_u)$, and $R_\textbf{P}$ are defined in Section \ref{iidr}.


\begin{thm}\label{r_state_thm_converse_obfs}
	For the above r-states mode, if $\widehat{\textbf{X}}^{(n)}$ is the obfuscated version of $\textbf{X}^{(n)}$, and $\widetilde{\textbf{X}}^{(n)}$ is the anonymized version of $\widehat{\textbf{X}}^{(n)}$  as defined, and
	\begin{itemize}
		\item $m =cn^{\frac{2}{s(r-1)} +  \alpha}$ for $c>0$ and $\alpha>0$;
		\item $R_u^{(n)} \sim Uniform [0, a_n]$, where $a_n \triangleq c'n^{-\left(\frac{1}{s(r-1)}+\beta\right)}$ for $c'>0$ and $\beta>\frac{\alpha}{4}$;
	\end{itemize}
	then user $1$ has no privacy as $n$ goes to infinity.  In other words, there exists an algorithm for the adversary to produce the estimation of ${X_1(k)} $ such that for large enough $n$,
	\begin{align}
	\no  \forall k\in \mathbb{N}, \ \ \ P_e(1)\triangleq P\left(\overbrace{X_1(k)}  \neq X_1(k)\right)\rightarrow 0.
	\end{align}
\end{thm}



\subsection{Markov Chain Model}
In this section, users' data patterns are modeled using Markov chains and there are $r$ possibilities for users' data patterns. Similar to Section \ref{markov}, we assume $p_u(i)$'s are drawn independently from some continuous density function, $f_P(\textbf{p}_u)$, on the $(0,1)^{|F|-r}$ hypercube.  $\textbf{p}_u$, $f_P(\textbf{p}_u)$, and $R_\textbf{P}$ are defined in Section \ref{markov}.

Using the above observations, we can now repeat the same reasoning as the last sections to show the following theorem.


\begin{thm}\label{markov_thm_obfs}
	For the an irreducible, aperiodic Markov chain model, iff $\widehat{\textbf{X}}^{(n)}$ is the obfuscated version of $\textbf{X}^{(n)}$, and $\widetilde{\textbf{X}}^{(n)}$ is the anonymized version of $\widehat{\textbf{X}}^{(n)}$  as defined, the size of a group is $s$, and
	\begin{itemize}
		\item $m =cn^{\frac{2}{s(|F|-r)} +  \alpha}$ for $c>0$ and $\alpha>0$;
\item $R_u^{(n)} \sim Uniform [0, a_n]$, where $a_n \triangleq c'n^{-\left(\frac{1}{s(|F|-r)}+\beta\right)}$ for $c'>0$ and $\beta>\frac{\alpha}{4}$;
	\end{itemize}
then the adversary will be able to single out all members of the group with arbitrary small error probability for large enough $n$. that is as $n \rightarrow \infty$,
	\begin{align}
	\no  \forall k\in \mathbb{N}, \ \ \ P_e(1)\triangleq P\left(\overbrace{X_1(k)}  \neq X_u(k)\right)\rightarrow 0.
	\end{align}
\end{thm}


\section{Achieving Perfect Privacy in the Presence of Correlation }
\label{perfect}
In the first part of the paper, we argue that the correlation could be disastrous to our privacy.  We proved independent obfuscation alone cannot be sufficient even if we use a high noise level.

In this part, we want to show how we can achieve perfect privacy in the presence of correlation. The problem is that the adversary can still reconstruct the association graph with small number of adversary's observations even if you add independent noise.  As a result, the connected users can collaborate together to increase their privacy.


For clarity of exposition, we focus on the two-state model where the association graph consists of subgraphs with $s_i\leq 2$. Thus, there are some users that are connected together and there are also some isolated users.  Now, we state the following theorem:
\begin{thm}
\label{thm:noise}
For the  two-state model, if $\widehat{\textbf{X}}^{(n)}$ is the obfuscated version of $\textbf{X}^{(n)}$, $\widetilde{\textbf{X}}^{(n)}$ is the anonymized version of $\widehat{\textbf{X}^{(n)}}$, and the size of all subgraphs are less than $2$, there exist an anonymization/obfusation scheme such that for all $(i,j) \in E$, the asymptotic noise level for users $i$ and $j$ is at most
\[a_e(i,j)= \frac{\abs{\cov (X_1(k), X_2(k))}}{\max \{p_i, p_j, 1-p_i, 1-p_j\}},\]
to achive perfect perfect privacy for all users.
\end{thm}







==> relatedwork.tex <==


